FMAS: Fast Multi-Objective SuperNet Architecture Search for Semantic Segmentation

We present FMAS, a fast multi-objective neural architecture search framework for semantic segmentation. FMAS subsamples the structure and pre-trained parameters of DeepLabV3+, without fine-tuning, dramatically reducing training time during search. To further reduce candidate evaluation time, we use a subset of the validation dataset during the search. Only the final, Pareto non-dominated, candidates are ultimately fine-tuned using the complete training set. We evaluate FMAS by searching for models that effectively trade accuracy and computational cost on the PASCAL VOC 2012 dataset. FMAS finds competitive designs quickly, e.g., taking just 0.5 GPU days to discover a DeepLabV3+ variant that reduces FLOPs and parameters by 10$\%$ and 20$\%$ respectively, for less than 3$\%$ increased error. We also search on an edge device called GAP8 and use its latency as the metric. FMAS is capable of finding 2.2$\times$ faster network with 7.61$\%$ MIoU loss.

==> data/pascal/Latency/gen1.tex <==
miou | latency
87.33  |  202.483510
86.06  |  767.197666
66.72  |  909.889742
33.03  |  2189.173539

==> data/pascal/Latency/gen10.tex <==
miou | latency
87.33  |  202.483510
82.76  |  285.370486
79.87  |  306.404086
79.87  |  306.404086
77.85  |  316.148074
64.15  |  317.430462
60.68  |  373.952471
58.03  |  782.576421
51.91  |  893.569066
49.2  |  1768.434878
41.68  |  1861.364288
39.0  |  1894.432311
33.03  |  2189.173539

==> data/pascal/Latency/gen15.tex <==
miou | latency
87.33  |  202.483510
82.76  |  285.370486
69.88  |  287.910141
64.15  |  317.430462
60.68  |  373.952471
54.84  |  400.519828
54.16  |  884.336235
51.91  |  893.569066
49.26  |  1663.063123
49.2  |  1768.434878
41.68  |  1861.364288
39.0  |  1894.432311
33.03  |  2189.173539

==> data/pascal/Latency/gen20.tex <==
miou | latency
87.33  |  202.483510
82.76  |  285.370486
69.88  |  287.910141
64.15  |  317.430462
60.11  |  354.930411
54.84  |  400.519828
54.16  |  884.336235
51.91  |  893.569066
49.85  |  948.100820
46.84  |  955.852763
42.35  |  1174.494655
40.36  |  1414.974725
39.0  |  1894.432311
33.03  |  2189.173539

==> data/pascal/Latency/gen25.tex <==
miou | latency
87.33  |  202.483510
76.39  |  252.005054
69.88  |  287.910141
64.15  |  317.430462
60.11  |  354.930411
54.84  |  400.519828
54.16  |  884.336235
51.91  |  893.569066
49.85  |  948.100820
46.84  |  955.852763
40.61  |  1004.415432
40.36  |  1414.974725
39.0  |  1894.432311
39.0  |  1894.432311
36.94  |  2085.645316
33.03  |  2189.173539

==> data/pascal/Latency/gen5.tex <==
miou | latency
87.33  |  202.483510
86.56  |  311.847120
64.15  |  317.430462
55.73  |  964.459607
49.2  |  1768.434878
41.68  |  1861.364288
39.0  |  1894.432311
33.03  |  2189.173539

==> data/pascal/flops/gen1.tex <==
miou | flops
94.73039321601391  |  36.351668925
93.71856823563576  |  37.276528133
92.29656159877777  |  40.134753053
88.75128626823425  |  45.381840549
84.72239673137665  |  76.954762997
52.13344097137451  |  83.953622501
23.144185543060303  |  108.505169549

==> data/pascal/flops/gen10.tex <==
miou | flops
88.79601806402206  |  34.470018221
83.09638947248459  |  35.403132949
70.12160122394562  |  36.336247677
64.10020291805267  |  38.202477133
44.79489326477051  |  40.068706589
42.490071058273315  |  41.001821317
36.38373017311096  |  42.868050773
32.09467530250549  |  54.751301541
31.560862064361572  |  57.876716197
28.388887643814087  |  87.408817181
23.429834842681885  |  97.956993365
23.23516011238098  |  101.473052093
23.144185543060303  |  108.505169549

==> data/pascal/flops/gen15.tex <==
miou | flops
88.79601806402206  |  34.470018221
83.09638947248459  |  35.403132949
69.35168504714966  |  36.336247677
64.05494511127472  |  37.269362405
59.08367037773132  |  38.202477133
49.77145195007324  |  39.135591861
43.73425841331482  |  40.068706589
41.94079637527466  |  41.001821317
37.68210411071777  |  41.934936045
36.38373017311096  |  42.868050773
36.20660901069641  |  50.063179557
32.09467530250549  |  54.751301541
30.27714490890503  |  56.314008869
27.42530107498169  |  87.408817181
24.947768449783325  |  90.924875909
24.323934316635132  |  94.440934637
23.429834842681885  |  97.956993365
22.689616680145264  |  101.473052093

==> data/pascal/flops/gen20.tex <==
miou | flops
88.79601806402206  |  34.470018221
83.09638947248459  |  35.403132949
69.35168504714966  |  36.336247677
61.857014894485474  |  37.269362405
61.857014894485474  |  37.269362405
54.70222234725952  |  38.202477133
49.598515033721924  |  39.135591861
40.869343280792236  |  40.068706589
37.68210411071777  |  41.934936045
36.38373017311096  |  42.868050773
36.20660901069641  |  50.063179557
33.36183428764343  |  53.188594213
32.09467530250549  |  54.751301541
30.27714490890503  |  56.314008869
28.877228498458862  |  57.876716197
27.42530107498169  |  87.408817181
24.947768449783325  |  90.924875909
24.323934316635132  |  94.440934637
23.19629192352295  |  97.956993365
23.19629192352295  |  97.956993365
22.623717784881592  |  101.473052093

==> data/pascal/flops/gen5.tex <==
miou | flops
83.09638947248459  |  35.403132949
73.83483350276947  |  37.314483941
67.84400343894958  |  50.069962533
63.76161873340607  |  51.632669861
37.77977228164673  |  53.188594213
34.85891819000244  |  87.408817181
23.89236092567444  |  97.956993365
23.23516011238098  |  101.473052093
23.144185543060303  |  108.505169549

==> data/pascal/flopsParams/models.tex <==
miou | flops | params
22.623717784881592  |  101.473052093  |  38.004053
23.19629192352295  |  97.956993365  |  36.376973
23.19629192352295  |  97.956993365  |  36.376973
23.19629192352295  |  97.956993365  |  36.376973
23.773711919784546  |  94.440934637  |  34.749893
24.947768449783325  |  90.924875909  |  33.122813
27.42530107498169  |  87.408817181  |  31.495733
28.877228498458862  |  57.876716197  |  38.004053
29.715323448181152  |  83.892758453  |  29.868653
30.27714490890503  |  56.314008869  |  36.376973
32.09467530250549  |  54.751301541  |  34.749893
33.36183428764343  |  53.188594213  |  33.122813
35.75238585472107  |  80.376699725  |  28.241573
36.20660901069641  |  50.063179557  |  29.868653
36.38373017311096  |  42.868050773  |  36.376973
37.03598976135254  |  76.860640997  |  26.614493
37.68210411071777  |  41.934936045  |  34.749893
40.869343280792236  |  40.068706589  |  31.495733
42.62846112251282  |  73.344582269  |  24.987413
49.598515033721924  |  39.135591861  |  29.868653
52.110740542411804  |  69.828523541  |  23.360333
54.70222234725952  |  38.202477133  |  28.241573
61.857014894485474  |  37.269362405  |  26.614493
61.857014894485474  |  37.269362405  |  26.614493
67.14242398738861  |  66.312464813  |  21.733253
69.35168504714966  |  36.336247677  |  24.987413
83.09638947248459  |  35.403132949  |  23.360333
86.01552248001099  |  62.796406085  |  20.106173
88.79601806402206  |  34.470018221  |  21.733253
93.07795986533165  |  163.872718909  |  18.479093

==> data/pascal/params/gen1.tex <==
miou | params
96.07687182724476  |  20.106173
69.66521143913269  |  24.987413
52.13344097137451  |  29.868653
23.144185543060303  |  41.258213

==> data/pascal/params/gen10.tex <==
miou | params
91.3274459540844  |  20.106173
75.55332630872726  |  21.733253
66.70951247215271  |  23.360333
42.62846112251282  |  24.987413
37.56006956100464  |  28.241573
33.624887466430664  |  29.868653
28.50416898727417  |  31.495733
25.469380617141724  |  33.122813
24.338579177856445  |  34.749893
24.000394344329834  |  36.376973
23.17821979522705  |  38.004053
22.67279624938965  |  39.631133

==> data/pascal/params/gen15.tex <==
miou | params
95.57437226176262  |  18.479093
91.3274459540844  |  20.106173
75.55332630872726  |  21.733253
60.210347175598145  |  23.360333
42.62846112251282  |  24.987413
41.83255434036255  |  26.614493
36.05297803878784  |  28.241573
33.624887466430664  |  29.868653
27.911359071731567  |  31.495733
25.469380617141724  |  33.122813
24.338579177856445  |  34.749893
23.777544498443604  |  36.376973
23.17821979522705  |  38.004053
22.67279624938965  |  39.631133

==> data/pascal/params/gen20.tex <==
miou | params
93.07795986533165  |  18.479093
86.01552248001099  |  20.106173
67.14242398738861  |  21.733253
52.110740542411804  |  23.360333
42.62846112251282  |  24.987413
37.03598976135254  |  26.614493
35.75238585472107  |  28.241573
29.715323448181152  |  29.868653
27.911359071731567  |  31.495733
25.469380617141724  |  33.122813
23.773711919784546  |  34.749893
23.19629192352295  |  36.376973
22.683227062225342  |  38.004053
22.67279624938965  |  39.631133

==> data/pascal/params/gen5.tex <==
miou | params
91.3274459540844  |  20.106173
79.46573495864868  |  23.360333
69.66521143913269  |  24.987413
51.59064829349518  |  26.614493
44.130051136016846  |  29.868653
34.9389374256134  |  31.495733
31.846266984939575  |  33.122813
24.338579177856445  |  34.749893
23.144185543060303  |  41.258213
